Real-time Speech Summarization for Medical Conversations

In doctor-patient conversations, identifying medically relevant information is crucial, posing the need for conversation summarization. In this work, we propose the first deployable real-time speech summarization system for real-world applications in industry, which generates a local summary after every N speech utterances within a conversation and a global summary after the end of a conversation. Our system could enhance user experience from a business standpoint, while also reducing computational costs from a technical perspective. Secondly, we present VietMed-Sum which, to our knowledge, is the first speech summarization dataset for medical conversations. Thirdly, we are the first to utilize LLM and human annotators collaboratively to create gold standard and synthetic summaries for medical conversation summarization. Finally, we present baseline results of state-of-the-art models on VietMed-Sum. All code, data (English-translated and Vietnamese) and models are available online: https://github.com/leduckhai/MultiMed/tree/master/VietMed-Sum

==> tables_and_figs/19k.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{llccc}
\hline
Model & R-1 & R-2 & R-L \\ 
\hline
$\text{BARTpho}_{\text{syllable}}$ & 58.18 & 36.91 & 45.94 \\
$\text{BARTpho}_{\text{word}}$ & 57.23 & 36.17 & 44.94 \\
ViPubmedT5 & 58.38 & 37.43 & 46.13 \\
ViT5 & 59.42 & 38.69 & 47.47 \\
ViT5-vietnews & 58.08 & 37.13 & 46 \\
\hline
\end{tabular}
\caption{Model performance on Train 19k dataset.}
\label{tab:performance_train_19k}
\end{table}


==> tables_and_figs/20k.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{llccc}
\hline
Model & R-1 & R-2 & R-L \\ 
\hline
$\text{BARTpho}_{\text{syllable}}$ & 58.68 & 37.79 & 46.81 \\
$\text{BARTpho}_{\text{word}}$ & 58.84 & 38.13 & 46.8 \\
ViPubmedT5 & 59.72 & 39.12 & 47.77 \\
ViT5 &\textbf{ 60.56} & \textbf{39.72 }& \textbf{48.59} \\
ViT5-vietnews & 60.07 & 39.51 & 48.24 \\
\hline
\end{tabular}
\caption{Model performance on Train 20k dataset.}
\label{tab:performance_train_20k}
\end{table}


==> tables_and_figs/ASR_WERs.tex <==
\begin{table}
\centering
\begin{tabular}{|l|cc|cc|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{ASR Model}} & \multicolumn{2}{c|}{WER}         & \multicolumn{2}{c|}{NEER}         \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                           & \multicolumn{1}{c|}{dev}  & test & \multicolumn{1}{c|}{dev}  & test \\ \hline
w2v2-Viet                                        & \multicolumn{1}{c|}{25.9} & 29.0 & \multicolumn{1}{c|}{25.4} & 28.3 \\ \hline
XLSR-53-Viet                                     & \multicolumn{1}{c|}{25.7} & 28.8 & \multicolumn{1}{c|}{25.2} & 27.9 \\ \hline
\end{tabular}
\caption{abcxyz}
\label{ASR_WERs}
\end{table}

==> tables_and_figs/LM_stats.tex <==
\begin{table*}
\centering
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Pre-trained LM}} & \multicolumn{1}{c|}{\textbf{\#Params}} & \multicolumn{1}{c|}{\textbf{\#Pre-trained Data}} & \multicolumn{1}{c|}{\textbf{\#Fine-tuned Data}} \\ \hline
ViT5-Base                                     &                                        &                                                  &                                                 \\ \hline
ViT5-Large                                    &                                        &                                                  &                                                 \\ \hline
mT5-Base                                      &                                        &                                                  &                                                 \\ \hline
mT5-Large                                     &                                        &                                                  &                                                 \\ \hline
Bartpho-Base                                  &                                        &                                                  &                                                 \\ \hline
Bartpho-Large                                 &                                        &                                                  &                                                 \\ \hline
mBART-Base                                    &                                        &                                                  &                                                 \\ \hline
mBART-Large                                   &                                        &                                                  &                                                 \\ \hline
ViHealthBERT-Base                             &                                        &                                                  &                                                 \\ \hline
ViHealthBERT-Large                            &                                        &                                                  &                                                 \\ \hline
ViPubmedT5-Base                               &                                        &                                                  &                                                 \\ \hline
ViPubmedT5-Large                              &                                        &                                                  &                                                 \\ \hline
\end{tabular}%
}
\caption{abcxyz}
\label{LM_stats}
\end{table*}

==> tables_and_figs/interannotator.tex <==
\begin{table}
\centering
\begin{tabular}{|l|l|l|l|}
\hline
                             & \multicolumn{1}{c|}{R1} & \multicolumn{1}{c|}{R2} & \multicolumn{1}{c|}{RL} \\ \hline
ChatGPT =\textgreater Human1 &       61.80                  &           44.27              &       50.10                  \\ \hline
% Human1 =\textgreater Human2  &         77.03                &             64.59            &         68.92               \\ \hline
ChatGPT =\textgreater Human2 &         55.20                &           59.74              &        59.77                 \\ \hline
\end{tabular}
\caption{abcxyz}
\label{interannotator}
\end{table}

% {'rouge1': 0.618006328074292, 'rouge2': 0.4427378731361159, 'rougeL': 0.5009887981375938, 'rougeLsum': 0.5019355595564368}
% {'rouge1': 0.7702936216789038, 'rouge2': 0.6459009358234469, 'rougeL': 0.689176705943831, 'rougeLsum': 0.6893173958595801}
% {'rouge1': 0.6909012247246341, 'rouge2': 0.552017335368494, 'rougeL': 0.5973993210233874, 'rougeLsum': 0.5977629115749494}


==> tables_and_figs/train_30s.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{llccc}
\hline
Model & R-1 & R-2 & R-L \\ 
\hline
 $\text{BARTpho}_{\text{syllable}}$ & 57.14 & 36.12 & 45.16 \\
 $\text{BARTpho}_{\text{word}}$ & 55.09 & 34.88 & 43.85 \\
 ViPubmedT5 & 58.26 & 36.12 & 45.9 \\
 ViT5 & 58.43 & 37.04 & 46.55 \\
 ViT5-vietnews & \textbf{59.49} & \textbf{37.98} & \textbf{47.21 }\\
\hline
\end{tabular}
\caption{Model performance on Train 30s dataset.}
\label{tab:performance_train_30s}
\end{table}

